Online Active Linear Regression via Thresholding

We consider the problem of online active learning to collect data for regression modeling. Specifically, we consider a decision maker with a limited experimentation budget who must efficiently learn an underlying linear population model. Our main contribution is a novel threshold-based algorithm for selection of most informative observations; we characterize its performance and fundamental lower bounds. We extend the algorithm and its guarantees to sparse linear regression in high-dimensional settings. Simulations suggest the algorithm is remarkably robust: it provides significant benefits over passive random sampling in real-world datasets that exhibit high nonlinearity and high dimensionality --- significantly reducing both the mean and variance of the squared error.

==> sections/related.tex <==
\section{Related Work}
\label{related}



% general
Active learning was formally defined in \cite{cohn1996active}, where optimal training data selection rules for neural networks, mixtures of Gaussians, and locally weighted regression models were proposed.
In \cite{cohn1994improving}, it was shown that, in some cases, the gain of active learning with respect to passive learning is exponential.
However, under worst-case distributional scenarios, active learning is no better than passive learning in terms of sample complexity, \cite{castro2007minimax, koltchinskii2010rademacher, balcan2010true}.

% classification
Active learning has been mainly studied for \emph{classification} problems in both realizable and agnostic settings.
Common approaches include disagreement-based techniques \cite{balcan2006agnostic, dasgupta2007general} where observations are chosen in regions where most hypotheses predict different outcomes, margin-based active learning \cite{balcan2007margin, wang2014noise} where algorithms aggressively query points close to the current decision boundary, and cluster-based algorithms \cite{dasgupta2008hierarchical}, which exploit a hierarchical tree-clustering of the unlabeled data.

% regression
Active learning in regression settings has been extensively explored too (see, e.g. \cite{krause2007nonmyopic, sugiyama2009pool, cai2013maximizing} and the references within).
The work in \cite{sabato2014active} focus on a setup similar to ours: online or stream-based active learning for linear regression with random design.
They propose a theoretical algorithm that partitions the space with a stratification technique based on Monte-Carlo methods, where a recently proposed algorithm for linear regression \cite{hsu2014heavy} is used as a black box.
It converges to the globally optimal oracle risk under possibly misspecified models under suitable assumptions.
% including that the total number of available observations (our $n$) is actually unlimited.

% more recent
Another relevant line of research is dynamic allocation of experimental units to treatment or control \cite{efron1971forcing}.
While randomized allocation is still the standard procedure, \cite{farias2015optimalabtesting} propose a novel tractable dynamic programming approach to A/B testing, where subjects are sequentially assigned to maximize the efficiency of the treatment effect estimate under linear model assumptions.
% The algorithm is able to compress a high-dimensional state space into a two-dimensional one when covariates come from elliptic distributions.
%The gain is most significant when the number of covariates and observations are similar, as balancing covariates becomes critical.


==> sections/ridge.tex <==
\section{Regularization}
\label{ridge}
Regularized linear estimators also benefit from large and balanced observations.
We show that, under certain mild assumptions, the performance of the Ridge estimator is directly aligned with that of previous sections: maximizing the minimum eigenvalue of the empirical covariance matrix.
Therefore, we expect Algorithm \ref{alg:threshold} to perform well under the Ridge estimator too.
While we do not theoretically study the Lasso estimator, for completeness, we perform extensive simulations with it in Section \ref{sim}.

The Ridge estimator is $\hat\beta_\lambda = \left( \X^T \X + \lambda I \right)^{-1} \ \X^T \y$, given $(\X, \y)$ and $\lambda > 0$.
\begin{theorem}
Let $R > 0$. Assume the penalty parameter for Ridge Regression is chosen uniformly at random $\lambda^* \sim U[0, R]$.
Then, the MSE of $\hat\beta_{\lambda^*}$ is upper bounded by
\begin{equation}
\E_{\lambda^*, \X} \ \| \hat\beta_{\lambda^*} - \beta^* \|^2 \le \E_{\X} \ f\left( \lambda_{\min}(\X^T\X) \right),
\end{equation}
where $f$ is the following decreasing function of $\lambda_{\min}$:
\begin{align*}
&f(\lambda_{\min}) = \frac{\sigma^2 \ d}{\lambda_{\min} + R} \\
&+ \| \beta^* \|^2_2 \left( 1 - \frac{2 \lambda_{\min}}{R} \log\left( 1 + \frac{R}{\lambda_{\min}} \right) + \frac{\lambda_{\min}}{\lambda_{\min} + R} \right).
\end{align*}
\end{theorem}
\begin{proof}
The proof is in the Appendix, Section F.
\end{proof}

==> sections/whitening.tex <==
\section{Whitening}
\label{whitening}
Before thresholding the norm of incoming observations, it is useful to decorrelate and standardize their components, i.e., to \emph{whiten} the data.
Then, we apply the algorithm to uncorrelated covariates, with zero mean and unit variance (not necessarily independent).
The covariance matrix $\Sigma$ can be decomposed as  $\Sigma = U D U^T$, where $U$ is orthogonal, and $D$ diagonal with $d_{ii} = \lambda_i(\Sigma)$.
We whiten each observation to $\bar{X} = D^{-1/2} U^T X \in \R^{d \times 1}$ (while for $\X \in \R^{k \times d}$, $\bar\X = \X U D^{-1/2}$), so that $\E \bar X \bar X^T = \mathrm{Id}$.
We denote whitened observations by $\bar X$ and $\bar \X$.
After some algebra we see that,
%\begin{equation} \label{eq:trace_white}
%\mathrm{Tr}(\Sigma(\X^T\X)^{-1}) = \mathrm{Tr}((\bar{\X}^T \bar{\X})^{-1}). 
%\end{equation}
%We trivially bound the previous expression as follows
%\begin{corollary}[derived from \cite{richter1958abschatzung}]\label{richter_coro}
%Let $A$ and $B$ be $n \times n$ Hermitian matrices, with $\lambda_1(A) \le \dots \le \lambda_n(A)$.
%Then,
%$\lambda_1(A) \ \mathrm{Tr}(B) \le \mathrm{Tr}(AB) \le \lambda_n(A) \ \mathrm{Tr}(B).$
%\end{corollary}
%We conclude, from \eqref{eq:trace_white} and Corollary \ref{richter_coro}, that
\begin{equation}\label{eq:trace_bound}
\frac{d}{\lambda_{\max}(\bar{\X}^T \bar{\X})} \le \mathrm{Tr}(\Sigma(\X^T\X)^{-1}) = \mathrm{Tr}((\bar{\X}^T \bar{\X})^{-1}) \le \frac{d}{\lambda_{\min}(\bar{\X}^T \bar{\X})}.
\end{equation}
Thus, we focus on algorithms that maximize the minimum eigenvalue of $\bar{\X}^T \bar{\X}$ with high probability, or, more generally, that lead to large and even eigenvalues of $\bar{\X}^T \bar{\X}$.
